Predictive Synthesis of API-Centric Code

Today's programmers, especially data science practitioners, make heavy use of data-processing libraries (APIs) such as PyTorch, Tensorflow, NumPy, Pandas, and the like. Program synthesizers can provide significant coding assistance to this community of users; however program synthesis also can be slow due to enormous search spaces. In this work, we examine ways in which machine learning can be used to accelerate enumerative program synthesis. We present a deep-learning-based model to predict the sequence of API functions that would be needed to go from a given input to a desired output, both being numeric vectors. Our work is based on two insights. First, it is possible to learn, based on a large number of input-output examples, to predict the likely API function needed in a given situation. Second, and crucially, it is also possible to learn to compose API functions into a sequence, given an input and the desired final output, without explicitly knowing the intermediate values. We show that we can speed up an enumerative program synthesizer by using predictions from our model variants. These speedups significantly outperform previous ways (e.g. DeepCoder) in which researchers have used ML models in enumerative synthesis.

==> daye_things_to_add.tex <==
Project Logs

Benchmarks

* Wrote PyTorch solutions for TF-coder’s StackOverflow, CoLab (https://www.internalfb.com/intern/anp/view/?id=690939), Google, Simple benchmarks.
* Collected 20 repair examples (https://docs.google.com/spreadsheets/d/10el5UA1lo6SWfJFVfYqkEQmZSLGNjbPhuR6BNlIA4OE/edit?usp=sharing) from StackOverflow
* Created a repair benchmark (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=328016812) containing 20 program repair examples. The repair examples collected from StakOverflow were too complicated to repair with our model, so I manually created wrong solutions of StackOverflow and Google benchmarks.
* Created a single-api benchmark (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=1049331683) containing 30 examples for a single-api prediction
* From StackOverflow benchmarks, removed examples that are out-of scope for the PyCoder+prediction model evaluation (link (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=328016812))
* Compared API n-gram frequences in benchmarks and general codebase (fbcode) (https://fb.quip.com/L8AAAs0bpZX4)
* Prediction model test benchmarks, containing input and output pairs that are not created by fuzzing (link (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=1575841497))
* Generative model test benchmarks to evaluate whether the model learned semantics, containing unseen sequences of APIs’ input and output (link (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=1526236489))

PyCoder Implementations

PyCoder currently does enumerative search following TF-Coder algorithm, except for the ML based prioritization. PyCoder models operation weights similar to TF-coder, by reusing the weights of corresponding Tensorflow functions, and does aggressive filtering with PyTorch specific filters. 
I submitted three diffs so far, and the first two are landed. Here is the summary of the PyCoder implementation updates.

* Updated TF-Coder implementation (https://github.com/google-research/tensorflow-coder) (diff1 (https://www.internalfb.com/diffs/browse?search_id=496293714825480&start=0&phabricator_diff_id=3505686442865815)) to work with PyTorch (diff2 (https://www.internalfb.com/diffs/browse?search_id=496293714825480&start=0&phabricator_diff_id=1412907855775359))
    * removed Tensorflow dependencies from all files
    * removed feature-based model
    * added a list of PyTorch tensor operations (torch_functions.py (https://www.internalfb.com/code/fbsource/fbcode/bigcode/archive/dayen/tensorflow-coder/tf_coder/torch_functions.py))
* Implemented filters for https://fb.quip.com/xueXAGmDmk89 (diff3 (https://www.internalfb.com/diffs/browse?search_id=940853733382570&start=0&phabricator_diff_id=1564196460578854))

After the mid-point review, I focused on incorporating prediction model into PyCoder. The Current PyCoder supports two ways of using the results of prediction models: 
1) Given input and output tensors, run prediction model before starting search, and reweight the operations based on the prediction results.
2) Run prediction before and during the enumerative search, with initial values, and values that are newly found through the search. No reweighting.
Another major addition was a snippet handler: to support program repair, I added an option to include attribute “snippet” in examples. “snippet” keeps the original PyTorch code to repair, and a snippet handler parses the snippet into AST, and reweight PyTorch operations and constants used in the original snippet search.
I submitted 11 diffs since mid-point review, and here is the summary of the PyCoder implementation updates.

* Program Repair
    * Repair benchmarks containing examples with original snippets (diff (http://d29462849/))
    * Snippet handler parsing the original snippet and reweight PyTorch operations in the original snippet in search (diff (http://d29520931/))
    * Multiplier reweighting constants (e.g., input tensor) used in the original snippet (diff (http://d29526305/))
* Incorporating prediction models
    * Single-api classification model + reweighting: before start searching, run single-api classification model with input tensor(s) and expected output tensor, and reweight top-n predicted operations lower (diff1 (http://d29618408/), diff2 (http://d29838727/), pseudo code (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge4f9b3ed6e_0_6))
    * Single-api classification model + iterative prediction: before starting the enumerative search using weights, run the prediction model with input values and check if there is a single api generating the expected output. If not, start the enumerative search, and for each new value found, run the prediction model with the new value. ( diff1 (http://d29681162/), diff2 (http://d29912700/), pseudo code (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge623ec09b2_0_0))
    * Single-api classification model + iteration by number of API calls: similar to Single-api + iterative prediction, but iterate the search space by the number of API calls, not by the weights (diff (http://d29717544/), pseudo code (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge4f9b3ed6e_0_12))
    * multi-api classification model: run multi-api classification model with input tensor(s) and expected output tensor, which returns a sequence of PyTorch operations. Given the sequence, PyCoder fills in argument values for each operation (diff (http://d29839026/), pseudo code (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge45d7c1a28_0_11))

*How to run PyCoder*
To run PyCoder, run 

buck run @mode/opt -c=python.package_style=inplace -j 8 bigcode/archive/dayen/tensorflow-coder/tf_coder:value_search_main

You can configure the followings:

* value_search_main.py
    * function run_on_all_benchmarks, change benchmarks to run
* value_search_settings.py
    * ModelSettings
        * use_multiplier: whether to use multiply model-predicted APIs before search
        * multiplier: reweight constant. [0, 1)
        * multiplier_top_n: the number of APIs to reweight, given a ranked list from prediction model
        * do_iterative_prediction: 
        * iterative_top_n: the number of APIs to evaluate for each prediction
        * threshold: softmax probability threshold
        * use_multi_model: whether to use multi-api prediction model
    * PrintSettings: 
    * 

Fuzzing

While analyzing PyCoder+prediction model results, I found that the initial fuzzing does not cover many patterns benchmarks. I listed up the missing patterns, read the initial fuzzing code, and improved them (notebook (http://n1009529/))

* 3 api call sequences were fuzzed only as api3(api2(api1)). 
* Initial fuzzing only used intermediate values (previous API call’s results) as their first arguments.
* There are operations takes both tensors and primitive values as their second arguments, but initial fuzzing supported only tensors for some operations (e.g., gt, eq, where).

*In the following 2 weeks:* Analyzing new training set will likely to give more patterns to cover, and I will update the fuzzing.

PyCoder Evaluation

The current version of PyCoder can synthesize 52% of examples in 300 seconds, on Google/StackOverflow benchmarks. Detailed benchmark results can be found here (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?usp=sharing).

* Out of 69 examples (after excluding ones with sparse-tensors),
    * 36 were correctly synthesized - took 30.00 seconds on average
    * 27 got timeout
    * 7 got caffe runtime errors (integer overflow) - WIP

*Single benchmarks:* To understand how well the single-api classification model works with PyCoder, we evaluted PyCoder + single-api model with single benchmarks. Detailed results can be found here (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=1049331683).

* Vanilla PyCoder: found 30 solutions out of 30 examples, in 4.24 sec/example.
* PyCoder + classification, reweighting operation weights to 1, using top-3 results: found 30 solutions out of 30 examples, in 0.89 sec / example.
* PyCoder + classification (trained with noise), reweighting operation weights to 1, using top-3 results: found 30 solutions out of 30 examples, in 0.55 sec / example.
* PyCoder + classification (trained with noise), reweighting operation weights to 1, using top-3 results, with threshold as 0.9 (confidence based on normalization, not using softmax): found 30 solutions out of 30 examples, in 0.73 sec / example.

*In-scope TF-coder StackOverflow benchmarks*: This is the benchmarks produced by TF-Coder authors, by collecting Tensorflow tensor manipulation examples from StackOverflow. I excluded out of scope examples, and now there are 37 examples. This is used to evaluate end-to-end performance of our models. Detailed results can be found here (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=1600062844).
(Note: I’ve updated vanilla PyCoder’s filtering system gradually, so current PyCoder could work better than the vanilla PyCoder results. Logging could have affected the time, so we’ll need to measure every model’s time again for the paper)

* Vanilla PyCoder: found 25 solutions out of 37, in 43.51 sec / example.
* PyCoder + iterative prediction (ver1): found 17 solutions out of 37, in 43.59 sec/example. Logged intermediate values to check the prediction results. Average time will be shorter without this logging. 3 out of 17 were found using prediction. Others were found via enumerative search.
* PyCoder + iterative prediction (ver2, with threshold and float model): found 19 solutions out of 37, in 4.66 sec/example. Logged intermediate values to check the prediction results. Average time will be shorter without this logging. 1 out of 19 were found using prediction. Others were found via enumerative search.
* PyCoder + iterative prediction (ver3, ver2 + predict with tensor values only, enumerate with primitive values only): found 27 solutions out of 37, in 67.07 sec/example. Logged intermediate values to check the prediction results. Average time will be shorter without this logging. 6 out of 27 were found using prediction. Others were found via enumerative search.
* PyCoder + multi-api prediction: found 2 solutions out of 37, in 0.79 sec/example. For multi-api prediction incorporation, I did not do operation search, so 35 examples were not timeout results, but wrong prediction.
* PyCoder + iteration by number of api calls: ran with 7 examples, and observed that it takes too long to search, so did not run with other examples and stopped evaluation.

Through the analysis, I could improve the iterative prediction, and find that initial fuzzing is not sufficient to train generalizable model. The analysis also showed the need of removing out-of-scope benchmarks, and using model confidence (probability).

*In the following 2 weeks:* In addition to the end-to-end evaluation, I will do measure local performance to evaluate how fuzzing affect the prediction model. For this evaluation, I will measure the precision of the prediction model, not the synthesis.

Program Repair

The original target application of PyCoder was to do program repair: given input tensors, desired output, and a snippet intended to create the expected output but does not, return a snippet that produces the desired output. I did implemented components to handle the snippet and search for the correct snippet, by prioritizing operations and values that are used in. the original snippet.
With repair benchmark (detailed results can be found here (https://docs.google.com/spreadsheets/d/1_YCzfGgwdsbwjlxW5jl--UJw214u3hM8VbBFv6QqT4U/edit?pli=1#gid=272021907)), 

* Vanilla PyCoder (synthesis from scratch): found 10 solutions out of 20, in 25.65 sec/example.
* PyCoder + reweighting operation: found 11 solutions out of 20, in 5.79 sec/example.
* PyCoder + reweighting operation and values: found 11 solutions out of 20, in 21.84 sec/example.

Current version of program repair does work with the benchmarks because they were created with an assumption that original snippet will be similar to the desired snippet. This is based on our reasoning that programmers writing PyTorch code will have reasonable knowledge on PyTorch and tensor manipulation. Therefore, this repair strategy will not work well with end users or programmers having no experience with machine learning. 
One bottleneck is the lack of benchmarks. Although I collected examples from StackOverflow, they usually don’t fit with our target use case. One idea to collect examples for the live coding repair scenario is to look at GitHub commits and extract updated snippets containing PyTorch operations.

User Interface (demo (https://drive.google.com/file/d/13_vdsM73Yhio1Tf-Wwg0xXj-zGqdqXeY/view?usp=sharing))

As PyCoder uses runtime values to synthesize code, live coding environment is potential environment to deploy PyCoder. 
To see the possibility of adding PyCoder to Bento Notebook, I explored LSPs and Wasabi code and implemented a simple demo. With a PyCoder Bento Kernel (diff (http://d29717306/)) and code I’ve wrote (haven’t committed as it changes Wasabi code - what will be the best way to share this code?), a user can get synthesized code Bento Notebook with the following steps:

* Assign an input tensor to a variable with any name (e.g., in1), and assign an output tensor into a variable named “output”, and run the cell
* In the next cell, type the input tensor name, and type a trigger character “[”, the synthesized snippet will show up in autocomplete  option lists. If no snippet shows up, that means PyCoder could not synthesize a solution.

The current version is not complete, but does show that it is possible to incorporate PyCoder into Bento Next. Due to the time constraints, I have not spend more time implementing the UI, but we hope to collaborate with the Bento team to finish this.
The target UI was:
cell n-1: in1 = ...
     in2 = ...
     out = ...
[run cell n-1]
cell n: out = in1, in2*?* --- [PyCoder] → out = [synthesized_code] (? is a trigger character)
For a better usability, we can provide a pop up where a user can type output tensor one by one after a trigger character, like skippy (slides (https://docs.google.com/presentation/d/1rPeykfUhCt40cGCg_u5jdApi9rPgM9BBqAzt2fCStTc/edit?usp=sharing)), or even to the cell directly, and while a user is typing the expected output, PyCoder can search gradually. 

code: update bento/wasabi/handler_functions/completion_functions.py with the following code


Findings and Ideas

* Findings from benchmark translation and PyCoder implementation is listed here (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit?usp=sharing)
* Some noteworthy ideas we came up with are
    * Repair problem definition (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge0b5e7445c_0_12)
        * When a programmer writes a wrong snippet, a programmer will more often get errors than wrong resulting values. Therefore, we want to focus on repairing snippets with errors.
    * Repair search strategy (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge117fb9cc7_0_0) (concrete example WIP (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gddeae741d1_0_6))
    * Search prioritization (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge0b5e7445c_0_17)
    * Additional sources of information in live coding setting (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gde82b1d339_0_336)
* Findings and ideas found the program repair, prediction model incorporation and UI implementation are listed here (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb800a09061_0_0), including:
    * Repair performance depends on the quality of the original snippet (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb800a09061_0_4)
    * Github commits can be used to built repair benchmarks (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb800a09061_0_19)
    * Some notes for the Wasabi development (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb81904e5ee_0_5)
    * Iterative prediction idea (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb81904e5ee_0_0)
    * Fuzzing (slide1 (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.ge45d7c1a28_0_16), slide2 (https://docs.google.com/presentation/d/157bBppYConH79Ro8ZB78hilY43leinp5zku_R6h00Lw/edit#slide=id.gb81904e5ee_0_5))

















- Do we need 50 APIs instead of just 25?

That's true.
You sent Today at 9:49 PM
But isn't that the issue with all the other classification problems?

Satish Chandra
sent Today at 9:50 PM
Yeah
You sent Today at 9:53 PM
I think we're not claiming that our model can learn the whole semantics of PyTorch, but we focus on showing the possibility of learning semantics. So increasing the number of supporting APIs efficiently can be our future work. I don't think this will reduce our contribution much, although I can see that the reviewer2 can nitpick about this.




- The concern will be that can we learn “semantics” for 50 apis together? 100?

If we can learn semantics for 25, I think we can do for 50.. The problem will be the confusing APIs - there are examples where the model got it right when there were fewer classes, but got it wrong when similar APIs were added. For example, the model got SO 37 right (tensordot), but got it wrong when mul is added. We cannot say that the model learned semantics, but it's also not showing that the model didn't learn semantics - because any of us who understand the semantics of tensordot and mul can get confused..?
You sent Today at 10:03 PM
So if we can come up with good models which can capture those subtle differences well, it will get less affected by the number of APIs. And I think coming up with a good model is the challenging part/




- order of input tensors matter

While I was debugging the pycoder end-to-end results, I found that the model is actually affected by the order of input tensors, even when it should not be. For example, for torch.add(in1, in2), the results should be same when we input (in1, in2) and (in2, in1), but the model correctly predicts add given (in1, in2), but not when it is given (in2, in1). It doesn't seem like the problem of fuzzing, because I randomly swap the order of tensors (in1 and in2).
You sent Today at 7:51 PM
Do you think this is expected by design..?

Satish Chandra
sent Today at 7:53 PM
This is so weird !
You sent Today at 8:07 PM
I'll try to investigate then. I don't know how often this occurs - maybe this is one in a million case.

Satish Chandra
sent Today at 8:10 PM
To me, this sounds like it might be learning to ignore one of the two (in1, in2).
Satish Chandra sent Today at 8:10 PM
Because some of the APIs have just one input, correct?
Satish Chandra sent Today at 8:10 PM
So may be training unary and binary APIs together is problematic?
You sent Today at 8:18 PM
oh that's actually a good point..

Satish Chandra
sent Today at 8:19 PM
Can you test out this hypothesis quickly?
You sent Today at 8:19 PM
this actually makes sense because this specific example is the one with larger range.
You sent Today at 8:20 PM
in1 is [100, 200, 300, 400] and 
in2 is [[[ 7,  9, 11, 13],
         [ 6,  7,  8,  9]],

        [[18, 23, 28, 33],
         [39, 50, 61, 72]]]
You sent Today at 8:20 PM
So when I try with (in1, in2), it predicts mul as the top-1, but when I try with (in2, in1), it predicts add.

Baishakhi Ray
sent Today at 8:22 PM
what happens if both values have shorter range
You sent Today at 8:23 PM
when I try with in1 = [1, 2, 3, 4] with the same in2, (in1, in2) returns mul, and (in2, in1) returns square - sqaure is unary tho
You sent Today at 8:26 PM
For this one, I kept the original output (107, 209, ...) just to see if the second input is ignored or not
You sent Today at 8:26 PM
If I try with in1 = [10, 20, 30, 40] with the same in2, and output = in1 + in2, both (in1, in2) and (in2, in1) predicts add as the top1
You sent Today at 8:27 PM
so it might be just the range issue..?

Satish Chandra
sent Today at 8:27 PM
How about you investigate with longer tensors?

Baishakhi Ray
sent Today at 8:27 PM
yeah, probably

Satish Chandra
sent Today at 8:27 PM
Like say 10 elements
You sent Today at 8:33 PM
so with the original range with 10 elements, (in1, in2) gives gather and (in2, in1) gives add
You sent Today at 8:33 PM
but the top-2 is add for the (in1, in2)

Satish Chandra
sent Today at 8:34 PM
Hmm. I wonder what the source of confusion is
You sent Today at 8:35 PM
Yeah originally, I thought the model is returning mul just by looking at the range of the output tensor, but there's something more complex happening



-fuzzing

* Updated APIs taking dim as parameters (max, squeeze, sum)
    * range of the dim parameter: [-len(size), len(size)-1]. So we used dim = random.choice(0, len(size)-1). in the original fuzzing. 
    * But it is also possible to not giving any dimension (e.g., torch.max(in1)), which behaves like dim=len(size). So I added this.


* Added scalar second input (eq, add, div, mul)
    * The original fuzzing supported this (e.g., add_scalar), but as the second argument was wrapped with torch.tensor, it was actually treated as a single-value tensor in the embedding.
* Updated broadcast 
    * The original broadcast didn’t generate some broadcastable sizes
        * e.g., given [7], it didn’t generate [7, 1] tensors (SO 06)
    * As we created the second input based on the first one, the second tensor tends to be smaller than the first one. So I swapped the in1 and in2 randomly
* Updated tensordot, gather fuzzing to be more general
* squeeze
    * when there’s no size 1 dimension, squeeze doesn’t do anything to the input. So I added size 1 dimension to the input tensor to make sure squeeze actually does something to the input.
* div
    * when there’s 0 in the second input, the output tensor contained inf, which made the training to return nan loss. I constrained the second input to not have 0
* bincount
    * added the limit of size
    * exclude max(in1) > MAX_SIZE 
* where
    * broadcast is possible
* bincount is flaky
* swapping the order of inputs could change the model prediction, even when it should not 

==> includes/includes.tex <==
%!TEX root = main.tex




% Table float box with bottom caption, box width adjusted to content
\usepackage{algorithm}
%\newfloatcommand{capbtabbox}{table}[][\FBwidth]
%\usepackage[dvipsnames]{xcolor}
\usepackage[font=small,labelfont=bf,tableposition=top]{caption}
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\usepackage[noabbrev]{cleveref}
\usepackage{boldline}
\usepackage{color,colortbl}
\usepackage{bigstrut}
% \usepackage[ruled]{algorithm2e}
\usepackage{amsmath,amsfonts}
\usepackage{amsmath}
\usepackage{array}
% \usepackage{algorithmic}
\usepackage{balance}
\usepackage{blindtext}
\usepackage{booktabs}
\usepackage{caption}
\usepackage[noabbrev]{cleveref}
%\usepackage{cite}
% \usepackage{color}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{eqparbox}
\usepackage{fancybox}
\usepackage{fancyvrb}
\usepackage{framed}
\usepackage{graphicx}
\usepackage{ifthen}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{multirow}
\usepackage{pifont}
\usepackage{stfloats}
\usepackage{subfig}
\usepackage{textcomp}
\usepackage{times}
\usepackage{url}
% \usepackage{xcolor}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{tabularx}
\usepackage[switch]{lineno}
\usepackage{ragged2e}

% \usepackage[switch]{lineno}
% \usepackage{lineno}
% \linenumbers

% \newcommand{\subparagraph}{}
\usepackage{titlesec}

\usepackage{tcolorbox}
\tcbuselibrary{listings,skins}
 
\usepackage{mathtools}
\usepackage{blindtext}
\usepackage{lstautogobble}

\usepackage{balance} 

\DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\graphicspath{{figures/}}



% spacing: how to read {12pt plus 4pt minus 2pt}
%           12pt is what we would like the spacing to be
%           plus 4pt means that TeX can stretch it by at most 4pt
%           minus 2pt means that TeX can shrink it by at most 2pt
%       This is one example of the concept of, 'glue', in TeX
\titlespacing{\section}{0pt}{8pt plus 4pt minus 2pt}{4pt plus 2pt minus 2pt}
 %\titlespacing{\section}{1pt}{\parskip}{-\parskip}
% \titlespacing{\subsection}{1pt}{\parskip}{-\parskip}
% \titlespacing{\subsubsection}{1pt}{\parskip}{-\parskip}

%\setlength{\belowcaptionskip}{-2mm}
%\setlength{\abovedisplayskip}{0pt}
%\setlength{\belowdisplayskip}{0pt}
%\setlength{\textfloatsep}{2pt}
%\setlength{\textfloatsep}{0.87\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}

% \renewcommand{\baselinestretch}{0.99}
%\captionsetup[table]{skip=1pt}
% \floatstyle{plaintop}
% \restylefloat{table}
\setlist{nolistsep}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.,}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.,}}\xspace}
\newcommand{\st}{\hbox{\emph{s.t.,}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace}
\newcommand{\vs}{\hbox{\emph{v.s.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}


\newtheorem{theorem}{Theorem}[section]
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\varname}[1]{{\small\texttt{#1}}\xspace}
%\newcommand{\tom}[1]{{\color{red} Tom: #1}\xspace}
\newcommand{\ch}[1]{{\color{black} #1}\xspace}
%\newcommand{\tableshrink}[1]{\vspace{-0.25in}}




\def\wv{\superscript{\S}}
\def\wu{$^{\dag}$}
\def\wg{\superscript{\ddag}}
\def\wn{$^{\natural}$}

\definecolor{gray50}{gray}{.5}
\definecolor{gray40}{gray}{.6}
\definecolor{gray30}{gray}{.7}
\definecolor{gray20}{gray}{.8}
\definecolor{gray10}{gray}{.9}
\definecolor{gray05}{gray}{.95}
\definecolor{gray01}{gray}{.97}

\newlength\Linewidth
\def\findlength{\setlength\Linewidth\linewidth
\addtolength\Linewidth{-4\fboxrule}
\addtolength\Linewidth{-3\fboxsep}
}
\newenvironment{examplebox}{\par\begingroup
  \setlength{\fboxsep}{3pt}\findlength
  \setbox0=\vbox\bgroup\noindent
  \hsize=0.90\linewidth
  \begin{minipage}{0.90\linewidth}\normalsize}
    {\end{minipage}\egroup
%    \vspace{6pt}
    \textcolor{gray20}{\fboxsep1.2pt\fbox
     {\fboxsep5pt\colorbox{gray05}{\normalcolor\box0}}}
%    \endgroup\par\addvspace{6pt minus 3pt}\noindent
    \endgroup\par\noindent
    \normalcolor\ignorespacesafterend}
\let\Examplebox\examplebox
\let\endExamplebox\endexamplebox

%-------------------------------------------------------------------------------------------
% Research Questions and Results
%
\newcounter{RQCounter}
\newcounter{RQACounter}

 %Pass in label for rq, then rq
%

% \newcommand{\RQ}[2]{%
% \refstepcounter{RQCounter} \label{#1}
%  \begin{center}	
%   \begin{examplebox}
%   \textbf{RQ\arabic{RQCounter}.}#2
%   \end{examplebox}	 
%  \end{center}
% }

% --- Material style Result Box ---
% \usepackage[framemethod=tikz]{mdframed}
\usetikzlibrary{shadows}
\usepackage{graphics}
\newmdenv[
    tikzsetting= {fill=blueish},
    skipabove=0.33em,
    skipbelow=0.33em,
    linewidth=1pt,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
    linecolor=gray95,
    roundcorner=2pt, 
    shadow=true,
    shadowsize=4pt,
    shadowcolor=gray95
]{questionbox}

\newmdenv[
    tikzsetting= {fill=greenish},
    skipabove=0.33em,
    skipbelow=0.33em,
    linewidth=1pt,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
    linecolor=gray95,
    roundcorner=2pt, 
    shadow=true,
    shadowsize=4pt,
    shadowcolor=gray95
]{answerbox}

\newmdenv[
    skipabove=0.33em,
    skipbelow=0.33em,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
]{lessonbox}

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,innersep=5pt] (char) {#1};}}
%\captionsetup{belowskip=3pt,aboveskip=3pt} % space between caption and content
\renewcommand\tabularxcolumn[1]{m{#1}} % tabularx align vertically
%\newcolumntype{s}{>{\centering \arraybackslash \hsize=.5\hsize}X}  % 

\newenvironment{lesson}
{
    \begin{lessonbox}
    Lessons Learned:\\
}
{\end{lessonbox}}




\newenvironment{result}
{\begin{answerbox}}
{\end{answerbox}}

\newenvironment{question}
{\begin{questionbox}}
{\end{questionbox}}



% \definecolor{javared}{rgb}{0.6,0,0} % for strings
% \definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
% \definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc

% \lstdefinestyle{basejava}{
%   language=java,
%   showstringspaces=false,
%   basicstyle=\small\ttfamily,
%   keywordstyle=\bfseries\color{javapurple},
%   commentstyle=\itshape\blue,
%   identifierstyle=\blue,
%   frame=none,
%   backgroundcolor=\color{white},
% }


% \lstdefinestyle{CustomJava}{
%   belowcaptionskip=\baselineskip,
%   breaklines=true,
%   xleftmargin=\parindent,
%   language=java,
%   showstringspaces=false,
%   basicstyle=\scriptsize\ttfamily,
%   keywordstyle=\bfseries\color{javapurple},
%   commentstyle=\itshape\blue,
%   identifierstyle=\blue,
%   belowskip=1pt,
%   frame=shadowbox,
%   backgroundcolor=\color{gray01},
%   gobble=0
% }


% \lstdefinestyle{codit}{
%   belowcaptionskip=\baselineskip,
%   breaklines=true,
%   %frame=single,
%   %xleftmargin=\parindent,
%   language=java,
%   showstringspaces=false,
%   basicstyle=\scriptsize\ttfamily,
%   keywordstyle=\bfseries\color{javapurple},
%   commentstyle=\itshape\blue,
%   identifierstyle=\blue,
% }

% \lstset{escapechar=@,style=customjava}
% \lstset{escapechar=@,style=codit}




% \newtcblisting{mylisting}[2][]{
%     %arc=0pt, outer arc=0pt,
%     %width=\columnwidth,
%     arc=3mm,
%     listing only, 
%     listing style=codit,
%     title=#2,
%     #1
%     }
    

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



% \usepackage{pythonhighlight}

\definecolor{Code}{rgb}{0,0,0} 
\definecolor{Decorators}{rgb}{0.5,0.5,0.5} 
\definecolor{Numbers}{rgb}{0.5,0,0} 
\definecolor{MatchingBrackets}{rgb}{0.25,0.5,0.5} 
\definecolor{Keywords}{rgb}{0.5,0,0.5} 
\definecolor{self}{rgb}{0,0,0} 
\definecolor{Strings}{rgb}{0,0.63,0} 
\definecolor{Comments}{rgb}{0,0.63,1} 
\definecolor{Backquotes}{rgb}{0,0,0} 
\definecolor{Classname}{rgb}{0,0,0} 
\definecolor{FunctionName}{rgb}{0.45,0.30,0.15} 
\definecolor{Operators}{rgb}{0,0,0} 
\definecolor{Background}{rgb}{0.98,0.98,0.98} 
 
\lstdefinelanguage{Python}{ 
    % numbers=left, 
    % numberstyle=\footnotesize\color{Numbers}, 
    % numbersep=1em, 
    xleftmargin=1em, 
    xrightmargin=1em,
    framextopmargin=0.5em, 
    framexbottommargin=0.5em, 
    showspaces=false, 
    showtabs=false, 
    showstringspaces=false, 
    frame=l, 
    tabsize=4, 
    % Basic 
    basicstyle=\ttfamily\small\setstretch{1}, 
    backgroundcolor=\color{Background}, 
    % Comments 
    commentstyle=\color{Comments}\slshape, 
    % Strings 
    stringstyle=\color{Strings}, 
    morecomment=[s][\color{Strings}]{"""}{"""}, 
    morecomment=[s][\color{Strings}]{'''}{'''}, 
    % keywords 
    morekeywords={import,from,class,def,for,while,if,is,in,elif,else,not,and,or,print,break,continue,return,True,False,None,access,as,,del,except,exec,finally,global,import,lambda,pass,print,raise,try,assert,len,tuple, list}, 
    keywordstyle={\color{Keywords}\bfseries}, 
    % additional keywords 
    morekeywords={[2]fuzz_sum}, 
    keywordstyle={[2]\color{FunctionName}\bfseries}, 
    emph={self}, 
    emphstyle={\color{self}\slshape}, 
    % 
} 


\usepackage[toc,page]{appendix}


\newcolumntype{d}[1]{D..{#1}}
\newcommand\mc[1]{\multicolumn{1}{c}{#1}}

% \setlength{\textfloatsep}{0pt plus 1.0pt minus 2.0pt}
% \setlength{\intextsep}{0pt plus 1.0pt minus 2.0pt}
% \setlength{\floatsep}{0pt plus 1.0pt minus 2.0pt}



==> includes/macros.tex <==
%!TEX root = main.tex
% This file is to define project specific macros

\newcommand{\ngm}{\$gram\xspace}
\newcommand{\ir}{$\mathscr{B}_{ir}$}
\newcommand{\ngmt}{\$gram+type\xspace}
%\newcommand{\sbfl}{SBBL\xspace}
\newcommand{\sbfl}{\hbox{${\cal S}\hspace{-0.01in}{\cal B}\hspace{-0.01in}{\cal B}\hspace{-0.01in}{\cal L}$}\xspace}
\newcommand{\LM}{\hbox{${\cal L}\hspace{-0.01in}{\cal M}$}\xspace}

\newcommand{\tool}{\textsc{PyCoder}\xspace}
\newcommand{\databug}{\textsc{Data from Charles Sutton}\xspace}

\newcommand{\review}[1]{\smallskip\noindent\textit{\textit{#1}}\smallskip}
\newcommand{\reponse}[1]{\noindent{#1\\}}

%% Response text prefix
\newcommand{\respto}[1]{
\fcolorbox{black}{black!15}{%
\label{resp:#1}%
\bf\scriptsize{\color{black}R{#1}}}\xspace%
}



%% Response text prefix
\newcommand{\bareresp}[1]{
\fcolorbox{black}{black!15}{%
\bf\scriptsize {\color{black}R{#1}}}\xspace%
}

% Cite responses
\newcommand{\citeresp}[1]{%
{(see }\fcolorbox{black}{black!15}{%
\bf\scriptsize R{#1}}~{{on page \pageref{resp:#1})}}}\xspace%

\newenvironment{response}
{\color{blue}}
{\color{black}}


\newcommand{\fus}{Full-Seq\xspace}
\newcommand{\fos}{First-Of-Seq\xspace}

\newcommand{\sts}{$\mathcal{S}2\mathcal{S}$\xspace}

\newcommand{\seq}{\sts}
\newcommand{\frontier}{{\tt frontier\_node}\xspace}

\newcommand{\Comment}[1]{}

\newcommand{\satish}[1]{{\todo{Satish:  {\color{red} #1}}}}
\newcommand{\daye}[1]{{\todo{Daye:  {\color{blue} #1}}}}
\newcommand{\rayb}[1]{{\todo{Baishakhi:  {\color{violet} #1}}}}
\newcommand{\sonia}[1]{{\todo{Sonia:  {\color{brown} #1}}}}
\newcommand{\amy}[1]{{\todo{Amy:  {\color{green} #1}}}}

\newcommand{\linecode}[1]{\lstinline[escapechar=@,basicstyle=\ttfamily]{#1}~}
\newcommand{\linecodewospace}[1]{\lstinline[escapechar=@,basicstyle=\ttfamily]{#1}}

\newcommand{\aucecen}{{\it {\bf $AUCEC_{en}$}}\space}
\newcommand{\aucecsp}{{\it {\bf $AUCEC_{sp}$}}\space}


% \newcommand{\rqa}{{\xspace How accurately \tool can suggest concrete edits?}\xspace}
% \newcommand{\rqa}{{\xspace How accurately can \tool suggest concrete edits?}\xspace}
% \newcommand{\rqb}{{\xspace How do different design choices affect \tool's performance?}\xspace}
% \newcommand{\rqc}{{\xspace How accurately \tool suggests bug-fix patches?}\xspace}

\newcommand{\treemodel}{$\mathscr{M}_{tree}$\xspace}
\newcommand{\tokenmodel}{$\mathscr{M}_{token}$\xspace}


\newcommand{\dataname}{\textit{Code-Change-Data}\xspace}
\newcommand{\icsedata}{\textit{Pull-Request-Data}\xspace}
\newcommand{\onelinetrain}{\textit{Bug-Repair-Data}\xspace}
\newcommand{\ktree}{$K_{tree}$\xspace}
\newcommand{\ktoken}{$K_{token}$\xspace}
\newcommand{\cross}{\ding{55}}
\newcommand{\tick}{\ding{51}}



%\newcommand{\citep}[1]{\cite{#1}}

\newcommand{\pcode}{$C_p$\xspace}
\newcommand{\ncode}{$C_n$\xspace}
\newcommand{\guidance}{$\mathcal{G}$\xspace}
\newcommand{\buggy}{$e_p$\xspace}
\newcommand{\fixed}{$e_n$\xspace}
\newcommand{\context}{$C$\xspace}


\newtcbox{\inlinebox}[1][]{enhanced,
 box align=base,
 nobeforeafter,
 colback=blueish,
 size=small,
 left=0pt,
 right=0pt,
 boxsep=2pt,
 #1}
 
% \newcommand{\highlight}[1]{
% \fcolorbox{black}{black!10}{%
% \footnotesize%
% \color{black}{%
% #1\xspace}}}%

\newcommand{\highlight}[1]{%
{\footnotesize%
\inlinebox{#1}%
}}

\newcommand{\sdata}{
{$B2F_{s}$}\xspace
}
\newcommand{\mdata}{
{$B2F_{m}$}\xspace
}



\newcommand{\rqa}{How accurately does \tool generate edited code \wrt other techniques?}
\newcommand{\rqb}{What  are  the  contribution  of  different  input  modalities in  \tool’s  performance?}
\newcommand{\rqc}{What  is  the  best  strategy  to  encode  multiple input  modalities?}

\newcommand{\RQrepeat}[2]{%
    \begin{question}{
    \small
    \noindent\textbf{RQ#1.~#2}
    }\end{question}
}

\newcommand{\RQ}[2]{%
    % \begin{question}
    {
    % \small
    \newline
    \refstepcounter{RQACounter} \label{rq-#1}
    \noindent\textbf{RQ\arabic{RQACounter}.~#2}
    \smallskip
    }
    % \end{question}
}

\newcommand{\RS}[2]{%
    \begin{result}
        \textbf{Result {\ref{rq-#1}}:~}{\emph {#2}}%
    \end{result}
}

\renewcommand{\cref}[1]{\Cref{#1}}

% \setlength{\belowcaptionskip}{-5pt}
\setlength{\abovecaptionskip}{-1pt}
\setlength{\intextsep}{3pt}
\setlength{\textfloatsep}{3pt}
\setlength{\dbltextfloatsep}{2pt}
\setlength{\textfloatsep}{2pt}
% \setlength{\dblfloatsep}{5pt}
% floatsep
% textfloatsep
% dbltextfloatsep
% dblfloatsep

\newcommand{\transBase}{{\em Transformer-base}\xspace}
\newcommand{\transLarge}{{\em Transformer-large}\xspace}

% \usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\makeatletter
\algrenewcommand\ALG@beginalgorithmic{\small}
\makeatother
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}


==> tables/intro_table.tex <==
\begin{table*}[t]
\footnotesize
 \caption{Example inputs/output and API calls. None of the predicted sequences are seen in the training set of sequences, and neither was the data. 
    %\daye{SO45 is out of scope for 16-api trained model. Would it be better to run PyCoder with 33 model? Also, SO16 }
    }
    \label{tab:api_examples}
    \centering
    \resizebox{1.98\columnwidth}{!}{%
    \begin{tabular}{l|l|l|l|l}
    \toprule
    \textbf{Benchmark} &    \textbf{Input(s)} & \textbf{Output} & \textbf{Predicted Sequence (Rank) \& Synthesized Program}  & \textbf{Synthesis} \\ \midrule
     SO45     & \texttt{in1 = [1, 0, 1, 0, 1]} & \texttt{[[34, 12],} & FOS: \textbf{unsqueeze} (8), \textbf{roll} (2), \textbf{where} (.)
     %\daye{Baishakhi, could you fill up the ranks of SO45 and SO37? \textbf{\bf unsqueeze (), roll (), where ()}}
     & FOS: Not found\\
     & \texttt{in2 = [[12, 34],} & \ \ \ \  \texttt{[56, 78],} & Full: \textbf{[unsqueeze, roll, where] } (4)  & Full: 2.61 sec  \\ 
    & \texttt{\ \ \ \ \ \ [56, 78],} & \ \ \ \ \texttt{[54, 23],}  & \texttt{{\textbf{\color{javapurple}where}}({\textbf{\color{javapurple}unsqueeze}}(in1,1).bool(),\texttt{{\textbf{\color{javapurple}roll}}(in2,1,-1),in2)}} & \\
    & \texttt{\ \ \ \ \ \ [23, 54],} & \ \ \ \  \texttt{[76, 78],} &   %\todo{related sequences seen in training}
                                                                    & \\
    & \texttt{\ \ \ \ \ \ [76, 78],} & \ \ \ \  \texttt{[24, 42]]} & & \\ 
    & \texttt{\ \ \ \ \ \ [42, 24]]} &  & &  \\  \midrule
    % SO 16 - single API classification
     SO16 & \texttt{in1 = [[2, 5], [3, 0], [8, 7]]} & {\texttt{[[8, 20],}} & FOS: \textbf{unsqueeze} (2), \textbf{mul} (3)  & FOS: 1.25 sec \\
     & \texttt{in2 = [4, 10, 6]} & {\ \ \ \ \texttt{[30, 0],}} & Full:  \textbf{unsqueeze}, \textbf{mul} (1) & Full: 0.62 sec \\
     &                          & {\ \ \ \ \texttt{[48, 42]]}} & {\texttt{{\textbf{\color{javapurple}mul}}(in1, torch.{\textbf{\color{javapurple}unsqueeze}}(in2, 1))}}&  \\ \midrule
    
    % % % SO 37 - single API classification
    % SO37 & \texttt{in1 = [[[10,20,30],} & \texttt{[[[850, 1900], } & FOS:  \textbf{mul ()}, \textbf{sum ()}  & FOS: 0.17 sec \\
    %  & \texttt{\ \ \ \ \ [40, 50, 60]],} & \texttt{\ \ [1520, 2890]]]} & Full: \textbf{[mul}, \textbf{sum] ()} & Full: 0.3 sec \\
    %  & \texttt{\ \ \ \ \ [[12, 34, 56], } & &\texttt{{\textbf{\color{javapurple}sum}}({\textbf{\color{javapurple}mul}}(in1, in2))}  &  \\
    %  & \texttt{\ \ \ \ \ [78, 98, 76]]]} & & &  \\
    %  & \texttt{in2 = [5, 10, 20]} & &  \\ \midrule
     
    % % SO 17 - single API classification, range > 20
    SO17 & \texttt{in1 = [17, 32, 99]} & \texttt{[[17, 17],  } &FOS: \textbf{stack} (1)  & FOS: 0.11 sec \\
     & \texttt{} & \texttt{\ [32, 32], } & Full: \textbf{[stack]} (1) & Full: 0.7 sec \\
      & \texttt{} & \texttt{\ [99, 99]]} &\texttt{\textbf{\color{javapurple}stack}((in1, in1), 1))}  &  \\ 
    %  % SO 34 - single API classification, range > 20
    % \texttt{in1 = [3, 5, 10]} & \texttt{[[128, 236], } & \texttt{torch.tensordot(in1, in2, 1)} \\
    % \texttt{in2 = [[[1, 2], [3, 4]], } & \texttt{\ [344, 452]]}  & \textbf{tensordot} \\
    % \texttt{\ \ \ \ \ \ [[5, 6], [7, 8]], } & &  \\ 
    % \texttt{\ \ \ \ \ \ [[10, 20], [30, 40]]]} & &  \\ \midrule
    % SO 22 - single API classification, float
    % \texttt{in1 = [3.0, 1.0, 10.0]} & \texttt{[32.3, 42.2]} & \texttt{torch.matmul(in1, in2)} & \\
    % \texttt{in2 = [[0.6, 0.4], [0.5, 1.0], } & & \textrm{matmul}  &\\
    % \texttt{\ \ \ \ \ \ \ [3.0, 4.0]]} & & &\\ \midrule
    
 
    
% [76, 78], [42, 24]
    
    \bottomrule
    \end{tabular}
    }
   
\end{table*}
% \todo{beautify this table and drop some rows}





% \begin{table*}[]
% \footnotesize
%     \centering
%     \begin{tabular}{l|l|l|l}
%     \toprule
%         input(s) & output & code \& predicted sequence & related sequences \\ \hline
%     % SO 16 - single API classification
%     \texttt{in1 = [[2, 5], [3, 0],[8, -7]]} & \texttt{[[8, 20], [30, 0],} & \texttt{torch.mul(in1, torch.unsqueeze(in2, 1))} & \\
%      \texttt{in2 = [4, 10, -6]} & \texttt{\ [-48, 42]]} & \textrm{}{ unsqueeze, mul} & \\ \hline
%     % SO 37 - single API classification
%     \texttt{in1 = [[[1.0, 2.0, 3.0], } & \texttt{[[[8.5, 19.0], } & \texttt{torch.sum(torch.mul(in1, in2))} & \\
%      \texttt{\ \ \ \ \ \ \ \ [4.0, 5.0, 6.0]],} & \texttt{\ \ [15.2, 28.9]]]} & \textrm{mul, sum} & \\
%      \texttt{\ \ \ \ \ \ \ [[1.2, 3.4, 5.6], } & & & \\
%      \texttt{\ \ \ \ \ \ \ \ [7.8, 9.8, 7.6]]]} & & & \\
%      \texttt{in2 = [0.5, 1.0, 2.0]} & & & \\
%      \hline
%     % SO 17 - single API classification, range > 20
%     \texttt{in1 = [17, -32, 99]} & \texttt{[[17, 17],  } & \texttt{torch.stack((in1, in1), 1))} &\\
%      \texttt{} & \texttt{\ [-32, -32], } & \textrm{stack} &\\
%      \texttt{} & \texttt{\ [99, 99]]} & & \\ \hline
%      % SO 34 - single API classification, range > 20
%     \texttt{in1 = [3, 5, 10]} & \texttt{[[128, 236], } & \texttt{torch.tensordot(in1, in2, 1)} & \\
%     \texttt{in2 = [[[1, 2], [3, 4]], } & \texttt{\ [344, 452]]}  & \textrm{tensordot} &\\
%     \texttt{\ \ \ \ \ \ [[5, 6], [7, 8]], } & & & \\ 
%     \texttt{\ \ \ \ \ \ [[10, 20], [30, 40]]]} & & & \\ \hline
%     % SO 22 - single API classification, float
%     \texttt{in1 = [3.0, 1.0, 10.0]} & \texttt{[32.3, 42.2]} & \texttt{torch.matmul(in1, in2)} & \\
%     \texttt{in2 = [[0.6, 0.4], [0.5, 1.0], } & & \textrm{matmul}  &\\
%     \texttt{\ \ \ \ \ \ \ [3.0, 4.0]]} & & &\\ \hline
    
%     \texttt{in1 = [1, 0, 1, 0, 1]} & \texttt{[[34, 12],} &
%     \texttt{torch.where(torch.unsqueeze(in1, 1).bool(), } & \\
%     \texttt{in2 = [[12, 34],} & \texttt{[56, 78],} & \texttt{    torch.roll(in2, 1, -1), in2)} & \\ 
%     \texttt{      [56, 78],} & \texttt{[54, 23],}  & \textrm{\bf unsqueeze, roll, where}& \\
%     \texttt{      [23, 54],} & \texttt{[76, 78],} & & \\
%     \texttt{      [76, 78],} & \texttt{[24, 42]]} & & \\ 
%     \texttt{      [42, 24]]} &  &  & \\ \hline
    
% % [76, 78], [42, 24]
    
%     \bottomrule
%     \end{tabular}
%     \caption{Examples of inputs/output and expected API calls. None of the predicted sequences were seen in the training set of sequences, and neither was the data.}
%     \label{tab:api_examples}
% \end{table*}
%  \todo{beautify this table and drop some rows}
